Parallel Weighted Model Counting with Tensor Networks

A promising new algebraic approach to weighted model counting makes use of tensor networks, following a reduction from weighted model counting to tensor-network contraction. Prior work has focused on analyzing the single-core performance of this approach, and demonstrated that it is an effective addition to the current portfolio of weighted-model-counting algorithms. In this work, we explore the impact of multi-core and GPU use on tensor-network contraction for weighted model counting. To leverage multiple cores, we implement a parallel portfolio of tree-decomposition solvers to find an order to contract tensors. To leverage a GPU, we use TensorFlow to perform the contractions. We compare the resulting weighted model counter on 1914 standard weighted model counting benchmarks and show that it significantly improves the virtual best solver.

==> unused.tex <==
\section{Trash}
\begin{definition}
Let $G$ be a graph. A \emph{contraction-sequence} of $G$ is a permutation $\pi = (e_1, \cdots, e_{|E(G)|})$ of the edges of $G$. Associated to each edge contraction sequence $\pi$ is a sequence of minors of $G$, denoted $\pi(G) = (G_1, \cdots, G_{|E(G)|+1})$, of length $|E(G)| + 1$ such that $G_1 = G$ and $G_{i+1}$ is obtained by contracting edge $e_i$ in $G_{i}$. The \emph{width} of a contraction sequence $\pi$ is the maximum degree seen across all vertices of all graphs of $\pi(G)$.
\end{definition}


% from http://iopscience.iop.org/article/10.1088/1751-8121/aa6dc3/pdf     % Tensors are a generalization of vectors and matrices. A $d$-dimensional vector can be considered an element of $\mathbb{C}^d$, and a $n \times m$-dimensional matrix an element of $\mathbb{C}^{n \times m}$. Correspondingly a rank-$r$ tensor of dimensions $d_1 \times \cdots \times d_r$ (which we will notate $\prod_{i} d_i$) is an element of $\mathbb{C}^{d_1 \times \cdots \times d_r}$. 

\begin{definition}
Let $T$ be a $d_1 \times \cdots \times d_r$-dimensional tensor, let $S$ be a $e_1 \times \cdots \times e_s$-dimensional tensor, and let $1 \leq a \leq r$ and $1 \leq b \leq s$ be indices into $T$ and $S$ with $d_a = e_b$. The \emph{contraction of $T$ and $S$ at $(a, b)$}, denoted $TS|^{a,b}$ is the rank-$(r+s-2)$ tensor of dimension $\prod_{i' \neq i} d_{i'} \times \prod_{j' \neq j} e_{j'}$ whose entry at position $(i_1, \cdots, i_{r+s-2})$ is given by
$$TS|^{a,b}_{i_1, \cdots, i_{r+s-2}} = \sum_{k=1}^{d_a} T_{i_1, \cdots, i_{a-1}, k, i_{a}, \cdots, i_{r-1}} S_{i_{r}, \cdots, i_{r+b-1}, k, i_{r+b}, \cdots, i_{r+s-2}}$$

\end{definition}

\begin{definition}
Let $T$ be a rank-$r$ tensor and $S$ be a rank-$s$ tensor over distinct indices, and let $a \in \ind{T}$ and $b \in \ind{S}$ be distinct indices with $|a| = |b|$. The \emph{contraction of $T$ and $S$ at $(a, b)$}, denoted $TS|^{a,b}$ is the rank-$(r+s-2)$ tensor with $\ind{TS|^{a,b}} = \ind{T} \cdot \ind{S} \setminus \{a, b\}$ whose entry at position $v$ is given by

$$TS|^{a,b}(v) = \sum_{k=1}^{|a|} T(v[a \mapsto k]) \cdot S(v[b \mapsto k])$$
\end{definition}
%In this work, for ease of notation we assume that every dimension of every tensor is fixed to a single size $d$ and so a rank-$r$ tensor is an element of $\mathbb{C}^{d^r}$.


\begin{definition}
A \emph{tensor} $T$ consists of
\begin{itemize}
\item a (finite, ordered) set $\ind{T} = \{i_1, \cdots, i_r\}$ of \emph{indices} of $T$, where each index $i \in \ind{T}$ has an associated finite \emph{domain} $[i]$, and
\item a function $T: [i_1] \times \cdots \times [i_r] \rightarrow \mathbb{C}$ that gives the value of the tensor for each possible assignment to the indices from elements of each domain.
\end{itemize}
The \emph{rank} of a tensor $T$ is $|\ind{T}|$.
\end{definition}




One fundamental binary operation on tensors is \emph{contraction}, which generalizes matrix multiplication to higher rank tensors.

\begin{definition}
Let $T$ and $S$ be tensors and enumerate $\ind{T} \cap \ind{S}$ as $\{i_1, i_2, \cdots, i_r\}$. The \emph{contraction product} of $T$ and $S$, denoted $T \cdot S$, is a tensor with $\ind{T \cdot S} = \ind{T} \oplus \ind{S}$ such that
$$(T \cdot S)(v) = \sum_{k_1, \cdots, k_r; 1 \leq k_j \leq |i_j|} T(v[i_j \mapsto k_j]) \cdot S(v[i_j \mapsto k_j])$$
\end{definition}

The notion of contraction product generalizes a variety of tensor operations. For example, if $T$ and $S$ share no indices their contraction product is exactly their tensor product. If $T$ and $S$ are matrices (i.e., rank 2 tensors) with a single shared index, then their product $T \cdot S$ is exactly the matrix obtained by multiplying $T$ and $S$ as matrices.

In this work, we are interested in computations that can be expressed as a sequence of contraction products. Since the tensor contraction product is commutative and (if every index appears at most twice across all tensors) associative, to specify such a computation it is enough to specify the set of tensors to contract.
\begin{definition}
A \emph{tensor contraction network} $\mathcal{M}$ is a set of tensors where every index appears at most twice. That is, every element of $\bigcup_{T \in M} \ind{T}$ has multiplicity 1 or 2. We call the elements of multiplicity 1 \emph{free indices} of $\mathcal{M}$ and notate the set of free indices of $\mathcal{M}$ by $\ind{\mathcal{M}}$.
\end{definition}

A tensor contraction network $\mathcal{M}$ uniquely identifies a tensor (which we will also denote for convenience by $\mathcal{M}$) with indices $\ind{\mathcal{M}}$ and whose value is given by computing the contraction product of all elements of $\mathcal{M}$ in an arbitrary order. The goal given a tensor contraction network $\mathcal{M}$ is to explicitly compute the tensor that $\mathcal{M}$ identifies.




Formally, a \emph{tensor network} is a set of tensors for which every index appears at most twice across all tensors. The problem of \emph{tensor network contraction}, given a tensor network $\mathcal{M}$, is to compute the tensor

One can check that this tensor product is commutative and associative, provided that every index appears at most twice across all tensors. 







A tensor network $(G, \mathcal{M})$ is a graph $G$, an implicit finite set of colors that can be used to label the edges of $G$, and a function $M_v \in \mathcal{M}$ for each vertex $v$ in the graph that maps each possible coloring of the edges incident to $v$ to a complex number. Thus for a given coloring $\ell$ of the edges of the graph, each vertex has an assigned value computed by $M_v$ (which we will denote by $M_v(\ell)$). The problem of \emph{tensor network contraction}, given a tensor network $(G, \mathcal{M})$, is to compute $\sum_{\ell \in L} \prod_{v \in V} M_v(\ell)$, where $L$ is the set of all edge colorings of $G$ and $V$ is the set of vertices of $G$. The notion of a tensor network captures many fundamental linear algebra concepts. 
% The problem of \emph{tensor network contraction}, given a tensor network $(G, \mathcal{M})$, is to compute $\sum_{\ell \in L} \prod_{v \in V} M_v(\ell)$, where $L$ is the set of all edge colorings of $G$ and $V$ is the set of vertices of $G$. Tensor network contraction is an important problem in a variety of fields, including 

\begin{lemma}
Let $N$ be a tensor contraction network and let $A$ and $B$ be distinct elements of $N$. Then $N' = (N \cup \{A \cdot B\}) \setminus \{A, B\}$ is also a tensor contraction network and $\tntensor{N} = \tntensor{N'}$.
\end{lemma}
\begin{proof} $N'$ is a tensor contraction network since $\dim{A \cdot B} \subseteq \dim{A} \cup \dim{B}$, and one can check that $\tntensor{N} = \tntensor{N'}$ by expanding the definition of $\tntensor{\cdot}$.
\end{proof}

One corollary of this result is, if $A$ and $B$ are distinct elements of a tensor contraction network $N$, then one can replace $A$ and $B$ with $A \cdot B$ in $N$ without changing the identified tensor. That is, $\tntensor{N} = \tntensor{(N \cup \{A \cdot B\}) \setminus \{A, B\}}$. 
We can therefore compute the tensor $\tntensor{N}$ represented by a tensor network $N$ by repeatedly contracting two elements of $N$ in an arbitrary order. Every stage of this computation produces a single intermediate tensor of some rank. Since for most dense representations of tensors the memory required is exponential in the rank, it is an important problem to find a sequence of contraction to perform to minimize the largest rank seen across all intermediate tensors.

\begin{definition}
Let $N$ be a tensor contraction network. A \emph{contraction sequence} for $N$ is a sequence of $|N|$ tensor networks $N_1 = N, N_2, \cdots, N_{|N|}$ such that each $N_{i+1}$ is obtained from $N_i$ by replacing two tensors with their contraction. That is, for every $1 \leq x < |N|$ there are $A_i, B_i \in N_i$ such that $N_{i+1} = (N_i \cup \{A_i \cdot B_i\}) \setminus \{A_i, B_i \}$.

The \emph{max-rank} of a contraction sequence $N_1, N_2, \cdots, N_{|N|}$ is the maximum rank across all tensors in every network.
\end{definition}

Note that a tensor contraction network can be specified in space polynomial in $|N|$ (without e.g. explicitly computing every tensor in the contraction sequence) by specifying at each $N_i$ the two tensors $A_i, B_i \in N_i$ to contract to form $N_{i+1}$.

Note that tensor networks containing a single tensor identify that tensor, i.e., $\tntensor{\{A\}} = A$ for all tensors $A$. A tensor network is closely related to the contraction operation: the union of two disjoint tensor networks $M$ and $N$ produces a tensor network that identifies $\tntensor{M} \cdot \tntensor{N}$. Formally:

% In order to prove the last part of Theorem 5, it will be more convenient to work with a alternative definition of branch-decomposition. Instead of labeling every leaf of the decomposition with an edge of $G$, we instead label every vertex of the decomposition with a (disjoint, possibly empty) subset of the edges of $G$.

% \begin{definition}
% Let $G$ be a simple graph. A \emph{generalized branch-decomposition} of $G$ is an unrooted binary tree $T$ together with a labeling function $\chi : L(T) \rightarrow 2^{E(G)}$ on the leaves of $T$ such that every edge of $G$ is contained in exactly one label of a node of $T$. That is, $V(G) = \bigcup_{n \in L(T)} \chi(n)$, and $\chi(n) \cap \chi(o) = \emptyset$ for all distinct $n, o \in L(T)$.

% As with a branch-decomposition, removing each arc $a \in E(T)$ partitions $T$ into two subgraphs $T_1$ and $T_2$. The union of the labels of the vertices of these subtrees, $L(T_1)$ and $L(T_2)$ are a partition of the leaves of $T$ and so are a partition of the edges of $G$; these sets of edges may share vertices in $G$. The \emph{width} of a generalized branch-decomposition is the maximum number of vertices incident both to an edge in $L(T_1)$ and an edge in $L(T_2)$ across all $a \in E(T)$. That is,
% $$width_b(T) = \max_{a \in E(T)} \left| \bigcap_{U \in CC(T \setminus a)} V(G \cap \bigcup_{n \in L(U)} \chi(n)) \right|.$$
% \end{definition}

% \begin{lemma}
% Let $G$ be a connected graph and let $w \geq 2$ be an integer. The following are equivalent:
% \begin{enumerate}
% \item There exists a branch-decomposition of $G$ of width $w$.
% \item There exists a nondegenerate generalized branch-decomposition of $G$ of width $w$.
% \end{enumerate}
% \end{lemma}
% \begin{proof}
% First, assume that $T$ is a branch-decomposition of $G$ of width $w$. Each leaf of $T$ is an edge of $G$, so let $\chi: L(T) \rightarrow 2^{E(G)}$ be the labeling function defined by $n \mapsto \{n\}$ for every $n \in L(T)$. The width of $(T, \chi)$, as a generalized branch-decomposition, is exactly the width of $T$. Finally, $(T, \chi)$ is nondegenerate since $|V(G \cap \chi(n)| = 2 \leq w$ for every $n \in L(T)$.

% Conversely, assume that $(T, \chi)$ is a nondegenerate generalized branch-decomposition of $G$ of width $w$. Construct a new generalized branch-decomposition $(T', \chi')$ by repeatedly performing the following: (1) remove from $T$ all leaves labeled with $\emptyset$, (2) label all newly created leaves with $\emptyset$, and (3) for every node $n$ in $T$ of degree 2, merge the two arcs incident to $n$ into a single arc and remove $n$ from $T$. Note that the width of $(T', \chi')$ is exactly the width of $(T, \chi)$, and moreover $(T', \chi')$ is nondegenerate since $(T, \chi)$ is. Finally, for each $n \in L(T')$, let $T_n$ be an (arbitrary) binary tree with leaves $\chi'(n)$. Construct $T''$ from $T'$ by attaching $T_n$ in place of each $n \in L(T')$. Since the labels of the leaves of $(T', \chi)$ partition $E(G)$, $L(T'') = E(G)$ and so $T''$ is a branch-decomposition of $G$. Moreover, the width of $T''$ is exactly the width of $(T', \chi)$; removing an arc in $T_n$ produces a decomposition with small width since $(T', \chi')$ is nondegenerate.
% \end{proof}

%Edges in $Line(G)$ are associated with vertices of $G$ (in particular, every vertex of $G$ produces a clique in $Line(G)$). We can attempt to produce a carving-decomposition from $T$ by replacing every $Line(G)$-edge on the leaves of $T$ with the corresponding $G$-vertex. Each vertex in $G$ can appear many times in this new carving-decomposition; if a single vertex appears far apart in this new carving-decomposition, its width may be dramatically higher than the width of $T$. Instead, we first modify $T$ to bring edges that correspond to the same vertex of $G$ close together. We show that we can do this without changing the width of $T$ since $Line(G)$ is a line graph. 


% \subsection{Appendix}

% \begin{lemma} \label{lemma:carving-to-contraction} Let $G$ be a graph. If $(T, \chi)$ is a carving-decomposition of $G$, then we can construct in polynomial time a contraction-sequence of $G$ whose width is no greater than the width of $(T, \chi)$.
% \end{lemma}
% \begin{proof}
% Choose arbitrarily a root for $T$, and at each internal node of $T$ arbitrarily denote the left child and the right child.
% \end{proof}

% \begin{lemma} \label{lemma:carving-to-branch} Let $G$ be a graph. If $T$ is a carving-decomposition of $G$, then we can construct in polynomial time a branch-decomposition $T'$ of $Line(G)$ such that $width_c(T) = width_b(T')$.
% \end{lemma}
% \begin{proof}
% For each vertex $v \in V(G)$, let $Clique(v) \subseteq V(Line(G))$ denote the set of vertices of $Line(G)$ corresponding to edges incident to $v$ in $G$. Note that $Clique(v)$ forms a clique in $Line(G)$, and in particular is associated to a set of edges in $Line(G)$. Construct a binary tree whose leaves are this set of edges in an arbitrary way; call it $T'(v)$ .

% We can then construct an unrooted binary tree $T'$ from $T$ by attaching, in place of each leaf $v$ of $T$, the binary tree $T'(v)$. $T'$ is still acyclic (since every edge in $Line(G)$ is in exactly one $Clique(v)$), and further the leaves of $T'$ are exactly the edges of $Line(G)$. Thus $T'$ is indeed a branch-decomposition of $Line(G)$; it remains to compute its width.

% To do this, consider an arc $a \in T'$. Either $a$ came from an arc in the original carving decomposition, or $a$ came from $T'(v)$ for some $v \in V(G)$. 
% \begin{itemize}
% \item If $a$ was an arc in the original carving decomposition, 
% $(v, w) \in V(Line(G))$ is incident to $L(T'_a)$ if and only if $v \in L(T_a)$ or $W \in L(T_a)$. Similarly, $(v, w) \in V(Line(G))$ is incident to $L(T' \setminus T'_a)$ if and only if $v \in L(T_a)$ or $W \in L(T_a)$. It follows that the width of $a$ in $T'$ is exactly the width of $a$ in $T$.
% \item Otherwise, $a$ is part of $T'(v)$ for some $v \in V(G)$. WLOG let $T'_a$ be the subtree of $T'(v)$. Then $(x, y) \in V(Line(G)$ is incident to an edge in $L(T'_a)$ if and only if $X = v$ or $y = v$. It follows that there the set of nodes of $Line(G)$ incident to an edge in $L(T'_a)$ is a subset of the edges incident to $v$ in $G$, and so the width of $a$ in $T'$ cannot be more than the degree of $v$ in $G$. Since the carving-width of $G$ is bounded from below by the maximum degree of $G$, it follows that the width of $a$ in $T'$ is no more than the width of $T$.
% \end{itemize}
% \end{proof}



% For each arc $(n, o) \in E(T)$, one element of $CC(T \setminus (n, o))$ contains $n$ and the other element contains $o$; let $T_{n,o}$ denote the element that contains $n$ and let $T_{o,n}$ denote the element that contains $o$.

% Define a partial order $\leq$ on the nodes of $T$ such that, for all $n, o \in T$,
% $$n \leq o~\text{if and only if}~I(G, \{v\}) \subseteq V(Line(G) \cap L(T_{o,n})).$$
% Intuitively, $n \leq o$ if and only if the ``$o$-component'' of $T \setminus \edge{o,n}$ contains ``enough'' edges in $Line(G)$ from the clique corresponding to $v$.

% \begin{enumerate}
% \item \textbf{Claim:} If $(n, o) \in E(T)$, then either $n \leq o$ or $o \leq n$ (or both).

% \textbf{Proof:} Assume that $n \not\leq o$. Thus there is some edge $\edge{v, w} \in I(G, \{ v \})$ that is not in $V(Line(G) \cap L(T_{o,n}))$. Since $L(T_{o,n})$ and $L(T_{n,o})$ partition $E(Line(G))$, $L(T_{n,o})$ must contain all edges of $Line(G)$ incident to $\edge{v, w}$. For every edge $\edge{v, x} \in I(G, \{ v \})$ there is an edge $e$ between $\edge{v, w}$ and $\edge{v, x}$ in $Line(G)$  and so $e$ must be in $L(T_o)$; it follows that $\edge{v, x} \in V(Line(G) \cap L(T_{n,o}))$. Hence $I(G, \{ v \}) \subseteq V(Line(G) \cap L(T_{n,o})$ and so $o \leq n$.

% \item \textbf{Claim:} If $n, o, p$ are distinct nodes in $T$, $\edge{p, o} \in E(T)$, and $o \leq n$, then $p \leq o$.

% \textbf{Proof:} Note that $o$ is on the shortest path from $p$ to $n$ and so $T_{n,o} \subseteq T_{o, p}$. Thus $L(T_{n,o}) \subseteq L(T_{o, p})$. It follows that $I(G, \{v\}) \subseteq V(Line(G) \cap L(T_{n,o})) \subseteq V(Line(G) \cap L(T_{o,p}))$.
% \end{enumerate}

% Given these two facts about the partial order $\leq$, we must find a ``maximal'' element of the partial order in $T$; we will then move all edges associated to the clique corresponding to $v$ to this location in the tree and show that the branch-width does not decrease.

% \begin{enumerate}
% \item[3.] \textbf{Claim:} There exists a node $n^*$ in $V(T)$ such that, for every neighbor $o$ of $n^*$, $o \leq n^*$.

% \textbf{Proof:} Assume for the sake of a contradiction that no such $n^*$ exists. For every $n \in V(T)$, we can therefore fix some neighbor $o(n)$ of $n$ such that $o(n) \not\leq n$. 
% Define a sequence of nodes of $T$ by $n_0 = n$ and $n_{i+1} = o(n_{i})$ for each $i \geq 1$, so that $n_{i+1} \not \leq n_i$. Since $T$ is a finite tree and each $n_{i+1}$ is a neighbor of $n_i$, we must eventually have $n_{j} = n_{j+2}$ for some $j \geq 0$. Thus $n_{j+1} \not\leq n_j$ and $n_j = n_{j+2} \not\leq n_{j+1}$, which contradicts the first claim above. 
% \end{enumerate}

%Since $V(T)$ is finite, there must be distinct $i, j > 0$ such that $n_i = n_j$. Thus $n_{i} \not\leq n_{j-1}$. By the first claim above, this implies $n_{j-1} \leq n_i$.  
%By the second claim above, since an edge exists between $n_{i}$ and $n_{j-1}$ this implies that $n_{i+1} \leq n_i$, a contradiction.
%Since $n_i \not \leq n_{i-1}$, $n_{i-1} \neq n_{j-1}$. If $n_{j-1} = n_{i+1}$, then $n_i \leq n_{i+1}$ and 
%By the second claim above, since an edge exists between $n_i$ and $n_{i+1}$ this implies that $n_{i+1} \leq n_i$, a contradiction.
%\end{enumerate}

% Every edge 

% For each vertex $v \in V(G)$, choose an arbitrary edge $e_v$ incident to $v$ in $G$. Let $E = \{ e_v : v \in V(G)\}$, so that we have $E \subseteq L(T)$. Let $S$ consist of the smallest connected subgraph of $T$ containing $E$, so that $L(S) = E$.

% Consider an arbitrary arc $a$ of $S$ and note that $a$ is also an arc of $T$. In particular, the leaf nodes of each element of $CC(S \setminus a)$ is a subset of the leaf nodes of some element of $CC(T \setminus a)$. It follows that
% $$\bigcap_{U \in CC(S \setminus a)} V(G \cap L(U)) \subseteq \bigcap_{T \in CC(S \setminus a)} V(G \cap L(U))$$
% Next, construct $S'$ by replacing each leaf node $e_v$ in $S$ by $v$, so that $L(S') = V(G)$.


% Thus $T'$ is now a carving-decomposition of $G$; it remains to compute its width.

% Let $a$ be an arbitrary arc of $T'$. Note that $T'_a \subseteq T_a$. 
% Consider an arc $a$ of $T'$, and note that $a$ corresponds to an arc of $T$. Removing 

% \begin{itemize}
% \item[]
% \textbf{Claim:} Let $C_1$ and $C_2$ be a partition of $E(Line(G))$. For every edge $v \in V(G)$, either $I(G, \{ v \}) \subseteq V(Line(G) \cap C_1)$ or $I(G, \{ v \}) \subseteq V(Line(G) \cap C_2)$.

% \textbf{Proof:} Assume that $I(G, \{ v \}) \not\subseteq V(Line(G) \cap C_1)$, so there is some edge $\edge{v, w} \in I(G, \{ v \})$ that is not in $V(Line(G) \cap C_1)$. Since $C_1$ and $C_2$ partition $E(Line(G))$, $C_2$ must contain all edges of $Line(G)$ incident to $\edge{v, w}$. For every edge $\edge{v, x} \in I(G, \{ v \})$ there is an edge $e$ between $\edge{v, w}$ and $\edge{v, x}$ in $Line(G)$  and so $e$ must be in $C_2$; it follows that $\edge{v, x} \in V(Line(G) \cap C_2)$. Hence $I(G, \{ v \}) \subseteq V(Line(G) \cap C_2)$.
% \end{itemize}


\begin{itemize}
	\item[1.] \textbf{Claim:} If $a \in \E{T_i}$ and $\einc{T_i}{a} = \{n, o\}$, then either $n \leq o$ or $o \leq n$ (or both).
	
	\textbf{Proof:} Note that $a = \edge{n,o}$ is the only arc in $T_i$ between $n$ and $o$. Assume that $n \not\leq o$. Thus there is some edge $e \in \vinc{G}{v_i}$ of $G$ that is not in $\einc{\Line{G}}{\C{T_{i}}{a}{o}}$. Restating, this implies no element of $\vinc{\Line{G}}{e}$ is in $\C{T_{i}}{a}{o}$. Since $T_{i}$ is a branch-decomposition of $\Line{G}$, the sets $\C{T_{i}}{a}{o}$ and $\C{T_{i}}{a}{n}$ partition $\E{\Line{G}}$ and so $\vinc{\Line{G}}{e} \subseteq \C{T_{i}}{a}{n}$.
	
	By the definition of a line graph, for every $f \in \vinc{G}{v_i}$ with $e \neq f$ there is an edge $\E{\Line{G}}$ (in particular, in $C_i$) incident to both $e$ and $f$. Moreover, since the degree of $v_i$ is at least 2 we have $\vinc{\Line{G}}{e} \neq \emptyset$. It follows that $\vinc{G}{v_i} \subseteq \einc{\Line{G}}{\vinc{\Line{G}}{e}}$ and so $\vinc{G}{v_i} \subseteq \einc{\Line{G}}{\C{T_{i}}{a}{n}}$.
\end{itemize}


To do this, let us define a relation $\leq$ on the nodes of $T_i$ such that, for all $n, o \in T_i$, 
$$n \leq o~\text{if and only if, for all}~a \in \E{T_{i-1}}~\text{between}~n~\text{and}~o\text{,}~\vinc{G}{v_i} \subseteq \einc{\Line{G}}{\C{T_i}{a}{o}}.$$
Intuitively, $n \leq o$ if and only if there are ``enough'' edges of $\Line{G}$ past $o$ in $T_i$ so that $C_i$ appears in the induced partition. We aim to find a maximal element of this relation: some node $n^* \in \V{T_i}$ such that $o \leq n^*$ for all neighbors $o$ of $n^*$. 

Assume for the sake of a contradiction that no such $n^*$ exists, i.e., for every $m \in \V{T_i}$ there is some neighbor $o$ of $m$ in $T_i$ such that $o \not\leq m$. Let $n_1, n_2, n_3, \cdots$ be an infinite sequence of nodes of $T_i$ such that, for all $k > 1$, $n_{k+1}$ is an arbitrary neighbor of $n_k$ with $n_{k+1} \not\leq n_k$ (which by assumption must exist). Since $T_i$ is a finite tree and each node is a neighbor of the previous node, we must eventually have $n_\ell = n_{\ell+2}$ for some $\ell \geq 1$. Thus $n_\ell \not\leq n_{\ell+1}$ and $n_{\ell+1} \not\leq n_\ell$.

Let $a$ be the arc between $n_\ell$ and $n_{\ell+1}$. Since $n_\ell \not\leq n_{\ell+1}$, there is some edge $e \in \vinc{G}{v_i}$ of $G$ that is not in $\einc{\Line{G}}{\C{T_{i}}{a}{n_{\ell+1}}}$. Since $n_{\ell+1} \not\leq n_{\ell}$, there is some edge $f \in \vinc{G}{v_i}$ of $G$ that is not in $\einc{\Line{G}}{\C{T_{i}}{a}{n_{\ell}}}$. If $e = f$, consider another edge $g \in \vinc{G}{v_i}$ with $e \neq g$ (which exists since the degree of $v_i$ is at least 2). By definition of a line graph, there is an edge $e_{v_i, \{e, g\}}$ of $\Line{G}$ incident to $e$ and so $e_{v_i, \{e, g\}}$ cannot be in either $\C{T_{i}}{a}{n_{\ell+1}}$ or $\C{T_{i}}{a}{n_{\ell}}$. If $e \neq f$, by definition of a line graph there is an edge $e_{v_i, \{e, f\}}$ of $\Line{G}$ incident to both $e$ and $f$ and so $e_{v_i, \{e, g\}}$ cannot be in either $\C{T_{i}}{a}{n_{\ell+1}}$ or $\C{T_{i}}{a}{n_{\ell}}$. In either case, this is a contradiciton since these sets partition $\E{\Line{G}}$.


\begin{definition}[Branch-Decomposition]
	Let $G$ be a simple graph. A \emph{branch-decomposition} of $G$ is an unrooted binary tree $T$ whose leaves are the edges of $G$, i.e. $\L{T} = \E{G}$. 
	
	Consider some $a \in \E{T}$ and let $\einc{T}{a} = \edge{m,n}$. Removing $a$ from $T$ partitions $T$ into two subtrees, one containing $m$ and one containing $n$. The leaves of these subgraphs, $\C{T}{a}{m}$ and $\C{T}{a}{n}$, are a partition of the leaves of $T$ and so are a partition of the edges of $G$; the number of vertices shared between these sets of edges is given by $|\einc{G}{\C{T}{a}{m}} \cap \einc{G}{\C{T}{a}{n}}|$. The \emph{width} of a branch-decomposition is the maximum number of vertices shared between these sets of edges across all $a \in \E{T}$. That is,
	$$width_b(T) = \max_{a \in \E{T}} \left| \bigcap_{n \in \einc{T}{a}} \einc{G}{\C{T}{a}{n}} \right|.$$
\end{definition}

\begin{lemma} \label{lemma:tree-to-branch} Let $H$ be a simple graph. If $(T, \chi)$ is a tree-decomposition of $H$, then we can construct in polynomial time a branch-decomposition $T'$ of $H$ such that $width_b(T') = width_t(T, \chi)+1$.
\end{lemma}
\begin{proof}
	Given in the proof of (5.1) in \cite{NS91}.
\end{proof}

\begin{lemma}
	\label{lemma:branch-to-carving-helper}
	Let $G$ be a graph and let $v \in \V{G}$ be a node of degree at least 2. If $T$ is a branch-decomposition of $\Line{G}$, we can construct in polynomial time a branch-decomposition $T'$ of $\Line{G}$ such that (1) $width_b(T) = width_b(T')$, (2) $C_v$ is induced by some partition of $T$, and (3) for every node $w \in \V{G}$, if $C_w$ (from Definition \ref{def:line-graph}) is induced by some partition of $T$ then $C_w$ is induced by some partition of $T'$.
\end{lemma}
\begin{proof}
	If $C_v$ is already induced by some partition of $T$, we are done. In particular, if the degree of $v$ is $2$ then $|C_v| = 1$ and so $C_v$ is induced by the arc incident in $T$ to the element of $C_v$. Otherwise, the degree of $v$ is more than 2 and we aim to construct $T'$ by moving all edges of $C_v$ close together without changing the induced partitions of other cliques. To do this, let us define a relation $\leq$ on the nodes of $T$ by, for all $n, o \in \V{T}$, 
	$$n \leq o~\text{if and only if, for all}~a \in \E{T_{i}}~\text{between}~n~\text{and}~o\text{,}~\vinc{G}{v} \subseteq \einc{\Line{G}}{\C{T}{a}{o}}.$$
	Intuitively, $n \leq o$ if and only if there are ``enough'' edges of $\Line{G}$ past $o$ in $T$ so that $C_v$ appears in the induced partition. We aim to find a maximal element of this relation: some node $n^* \in \V{T}$ such that $o \leq n^*$ for all neighbors $o$ of $n^*$. 
	
	Assume for the sake of a contradiction that no such $n^*$ exists, i.e., for every $m \in \V{T}$ there is some neighbor $o$ of $m$ in $T$ such that $o \not\leq m$. Let $n_1, n_2, n_3, \cdots$ be an infinite sequence of nodes of $T$ such that, for all $i > 1$, $n_{i+1}$ is an arbitrary neighbor of $n_i$ with $n_{i+1} \not\leq n_i$ (which by assumption must exist). Since $T$ is a finite tree and each node is a neighbor of the previous node, we must eventually have $n_j = n_{j+2}$ for some $j \geq 1$. Thus $n_j \not\leq n_{j+1}$ and $n_{j+1} \not\leq n_j$.
	
	Let $a$ be the arc between $n_j$ and $n_{j+1}$. Since $n_j \not\leq n_{j+1}$, there is some edge $e \in \vinc{G}{v}$ of $G$ that is not in $\einc{\Line{G}}{\C{T}{a}{n_{j+1}}}$. Since $n_{j+1} \not\leq n_{j}$, there is some edge $f \in \vinc{G}{v}$ of $G$ that is not in $\einc{\Line{G}}{\C{T}{a}{n_{j}}}$. If $e = f$, consider another edge $g \in \vinc{G}{v}$ with $e \neq g$ (which exists since the degree of $v$ is at least 2). By definition of a line graph, there is an edge $e_{v, \{e, g\}}$ of $\Line{G}$ incident to $e$ and so $e_{v, \{e, g\}}$ cannot be in either $\C{T}{a}{n_{j+1}}$ or $\C{T}{a}{n_{j}}$. If $e \neq f$, by definition of a line graph there is an edge $e_{v, \{e, f\}}$ of $\Line{G}$ incident to both $e$ and $f$ and so $e_{v, \{e, g\}}$ cannot be in either $\C{T}{a}{n_{j+1}}$ or $\C{T}{a}{n_{j}}$. In either case, this is a contradiction since these sets partition $\E{\Line{G}}$.
	
	Thus there is some $n^* \in \V{T}$ such that $o \leq n^*$ for all neighbors $o$ of $n^*$. Moreover, if $n$ 
	
	If there is some arc
\end{proof}



\begin{lemma} \label{lemma:branch-to-carving} Let $G$ be a graph. If $T$ is a branch-decomposition of $\Line{G}$, then we can construct in polynomial time a carving-decomposition $T'$ of $G$ such that $width_b(T) \geq width_c(T')$.
\end{lemma}
\begin{proof}
	Let $V_0$ be the set of vertices of $G$ of degree 0, let $V_1$ be the set of vertices $G$ of degree 1, and let $V_2$ be the set of vertices of $G$ of higher degree. Notice that the vertices in $G$ 
	
	
	of $G$ of degree 1 or 0 and let $V_2$ be the set of vertices of $G$ 
	Let us first assume that every vertex of $G$ of degree 1 is a neighbor of some vertex of higher degree. 
	
	
	For every vertex $v \in \V{G}$ let $B_v$ be an arbitrary 
	
	
	Recall from Definition \ref{def:line-graph} that, for each $v \in \V{G}$, $C_v$ is a clique of edges in $\Line{G}$. Note that $C_v$ is empty if the degree of $v$ is 0 or 1. Let $V$ be the set of vertices of $G$ of degree $2$ or more and enumerate $V$ arbitrarily as $v_1, v_2, \cdots, v_{|V|}$.
	
	We prove by induction on $i$ that there exists a sequence of branch-decompositions $T_0, T_1, \cdots, T_{|\V{G}|}$ of $\Line{G}$ such that: (1) the width of $T_i$ is equal to $T$, and (2) for every $1 \leq j \leq i$, $C_{v_j}$ is induced by some partition of $T_i$.
	
	In the base case, we take $T_0 = T$ so that both conditions trivially hold. In the inductive step, we apply Lemma \ref{lemma:branch-to-carving-helper} to $T_{i-1}$ and $v = v_i$ to obtain a branch-decomposition $T_i$ such that (1) $width_b(T_i) = width_b(T_{i-1}) = width_b(T)$, (2) $C_{v_i}$ is induced by some partition of $T_i$, and finally (3) $C_{v_j}$ is induced by some partition of $T_i$ (for all $1 \leq j < i$) since $C_{v_j}$ was induced by some partition of $T_{i-1}$. 
	
	It follows that $T_{|V|}$ is a branch-decomposition of $\Line{G}$ such that $width_b(T_{|V|}) = width_b(T)$ and, for every $v \in V$, $C_v$ is induced by some partition of $T_{|V|}$. 
\end{proof}


\begin{theorem} \label{thm:correspond}
	Let $G$ be a connected graph with $\E{\Line{G}} \neq \emptyset$ and let $w \in \mathbb{Z}$. The following are equivalent:
	\begin{enumerate}
		\item There exists a carving-decomposition of $G$ of width no more than $w$.
		\item There exists a tree-decomposition of $\Line{G}$ of width no more than $w+1$.
		\item There exists a branch-decomposition of $\Line{G}$ of width no more than $w$.
	\end{enumerate}
	Moreover, given one of these objects both of the others can be constructed in polynomial time. 
\end{theorem}
\begin{proof}
	Lemma \ref{lemma:carving-to-tree} proves that (1) implies (2). Lemma \ref{lemma:tree-to-branch} proves that (2) implies (3), since $\Line{G}$ is simple. Lemma \ref{lemma:branch-to-carving} proves that (3) implies (1).
\end{proof}

Notably, Theorem \ref{thm:correspond} also shows for line graphs that we can transform branch-decompositions into tree-decompositions of equivalent (or smaller) width. Every tree-decomposition of a simple graph can be transformed into a branch-decomposition of equivalent width, but the converse is not true for general simple graphs \cite{NS91}. It follows that the tree-width of line graphs is exactly 1 smaller than the branch-width. Note that line graphs can be recognized in linear time.

$\E{G \cap F} = F$, so that $\V{G \cap F} = \bigcup_{e \in F} \einc{G}{e}$, i.e., the set of vertices of $G$ incident to some edge in $F$. We further define $G \setminus F = G \cap (\E{G} \setminus F)$. We sometimes abbreviate $G\setminus \{a\}$ to $G\setminus a$, etc.  

A subgraph $G'$ of $G$ is a \emph{connected component} of $G$ if $G'$ is connected and $\E{G'}$ contains exactly the edges of $G$ incident to some vertex in $\V{G'}$. We use $CC(G)$ to denote the set of connected components of $G$, and note that the sets of vertices of the elements of $CC(G)$ form a partition of $\V{G}$.


Every vertex $v \in \V{G}$ is associated with a set $\vinc{G}{v} \subseteq \E{G}$ of incident edges, and every edge $e \in \E{G}$ is associated with a set $\einc{G}{e} \subseteq \V{G}$ of two incident vertices (so $|\einc{G}{e}| = 2$ for every $e \in \E{G}$). 


\begin{definition}[Carving-Decomposition]
	Let $G$ be a graph. A \emph{carving-decomposition} of $G$ is an unrooted binary tree $T$ whose leaves are the vertices of $G$, i.e. $\L{T} = \V{G}$. 
	
	Consider some $a \in \E{T}$ and let $\einc{T}{a} = \edge{m,n}$. Removing $a$ from $T$ partitions $T$ into two subtrees, one containing $m$ and one containing $n$. The leaves of these subgraphs, $\C{T}{a}{m}$ and $\C{T}{a}{n}$, are a partition of the leaves of $T$ and so are a partition of the vertices of $G$; the number of edges between these sets of vertices is given by $|\vinc{G}{\C{T}{a}{m}} \cap \vinc{G}{\C{T}{a}{n}}|$. The \emph{width} of a carving-decomposition is the maximum number of edges between these sets of vertices across all $a \in \E{T}$. That is,
	$$width_c(T) = \max_{a \in \E{T}} \left| \bigcap_{n \in \einc{T}{a}} \vinc{G}{\C{T}{a}{n}} \right|.$$
\end{definition}



Given this lemma, we can proceed to prove the first part of Theorem \ref{thm:contraction-equiv-carving}: that contraction-trees can be transformed into carving-decompositions.
\begin{lemma} \label{lemma:contraction-to-carving}
	Let $N$ be a tensor contraction network and structure graph $G$. Let $T$ be a contraction-tree for $N$ of max-rank $w$. Then we can construct in $O(|N|)$ time a carving-decomposition $T'$ of $G$ such that $width_c(T') = w$.
\end{lemma}
\begin{proof}
	Let $r$ be the root of $T$ and let $f$ be the free vertex of $G$. Construct $T'$ from $T$ by adding $f$ and adding an arc between $r$ and $f$. Thus $\V{T'} = \V{T} \sqcup \{n\}$, $\L{T'} = \L{T} \sqcup \{f\}$, and $T'$ is an unrooted binary tree. Moreover, $\L{T'} = N \sqcup \{f\} = \V{G}$ and so $T'$ is a carving-decomposition for $G$. 
    
    It remains to check that carving-width of $T'$ is $w$. For each $n \in \V{T}$, let $C_n$ denote the tensor contraction network associated to $n$ as in Definition \ref{def:contraction-tree}. Consider an arbitrary partition $C \in \P{T'}$ induced by an arc $a \in \E{T'}$; since we are interested in $|\vinc{G}{C} \cap \vinc{G}{\V{G} \setminus C}|$, we can assume WLOG that $f \not\in C$ (otherwise, replace $C$ with $\V{G} \setminus C$.
    
    \begin{itemize}
    	\item If $a$ is the new arc between $r$ and $f$, then $C = N$. Thus $\vinc{G}{C} \cap \vinc{G}{C} = \tnfree{N}$ and so $\left| \vinc{G}{C} \cap \vinc{G}{C} \right| = | \tnfree{N} | = \rank{C_r} \leq w$.
        \item Otherwise, $a$ is also an arc of $T$. Thus $C$ is also a partition induced by $T$, and in fact $C = C_n$ for some node $n \in \einc{T}{a}$. It follows that $|\tnfree{C}| \leq w$. Moreover, in this case $C \subseteq N$ and so by Lemma \ref{lemma:tcn-equiv-structure} $\tnfree{C} = \vinc{G}{C} \cap \vinc{G}{\V{G} \setminus C}$. It follows that $|\vinc{G}{C} \cap \vinc{G}{\V{G} \setminus C}| \leq w$.
    \end{itemize}
	In all cases, $\left| \vinc{G}{C} \cap \vinc{G}{\V{G} \setminus C} \right| \leq w$. Hence $width_c(T') \leq w$. If $\rank{N} = w$, considering partitions induced in $T$ by the new arc between $n$ and $f$ shows that $width_c(T') \geq w$ as well. Otherwise, $\rank{C_n} = w$ for some node $n \in \V{T}$. Since $C_n$ is induced by $T$ and the corresponding subtree does not contain $r$, $C_n$ is induced by $T'$. By Lemma \ref{lemma:tcn-equiv-structure}, $|\vinc{G}{C_n} \cap \vinc{G}{\V{G} \setminus C_n}| = w$ and thus $width_c(T') \geq w$. Hence $width_c(T') = w$ as desired.
\end{proof}

Finally, we prove the second part of Theorem \ref{thm:contraction-equiv-carving}: that carving-decompositions can be transformed into contraction-trees.
\begin{lemma} \label{lemma:carving-to-contraction}
	Let $N$ be a tensor contraction network with structure graph $G$. Let $T$ be a carving-decomposition of $G$ of carving-width $w$. Then we can construct in $O(|N|)$ time a contraction-tree $(T', a)$ of $N$ of max-width $w$.
\end{lemma}
\begin{proof}
	Let $f$ be the free vertex of $G$. Since $f$ is a leaf of $T$ there is a single arc $a$ incident to $f$. Let $r$ be the other node of $T$ incident to this arc. Construct $T'$ from $T$ by removing $f$ and $a$, so that $T'$ is a rooted binary tree with root $r$. Notice $\L{T'} = N$ and so $T'$ is indeed a contraction-tree of $N$. For each $n \in \V{T'}$, let $C_n$ denote the tensor contraction network associated to $n$ as in Definition \ref{def:contraction-tree}. It remains to check that the max-rank of $T'$ is $w$.
    
    First, notice that $C_r = N$ is a partition induced by $T$ at $a$. Thus $\rank{N} = |\tnfree{N}| = |\vinc{G}{N} \cap \vinc{G}{\{f\}}| \leq w$. Next, consider a non-root node $n \in \V{T}$. Then $C_n$ is a partition induced by $T'$ and the corresponding subtree does not contain $r$, so $C_n$ is also a partition induced by $T$. By Lemma \ref{lemma:tcn-equiv-structure}, it follows that $\rank{C_n} \leq |\vinc{G}{C_n} \cap \vinc{G}{\V{G} \setminus C_n}| \leq w$. Therefore the max-rank of $T'$ is no more than $w$.
    
    To show equality, note that there is some partition $C$ induced by $T$ with $|\vinc{G}{C} \cap \vinc{\V{G} \setminus C}| = w$. If $C = N$ or $C = \{f\}$, then $\rank(C_r) = |\tnfree{N}| = w$. Otherwise, either $f \not\in C$ or $f \not\in \V{G} \setminus C$ so either $C$ or $\V{G} \setminus C$ is also a partition induced by $T'$ whose corresponding subtree does not contain $r$. Thus $C = C_n$ for some $n \in \V{T}$. By Lemma \ref{lemma:tcn-equiv-structure}, $\rank{C_n} = |\tnfree{C_n}| = |\vinc{G}{C} \cap \vinc{G}{\V{G} \setminus C}| = w$. Thus the max-rank of $T'$ is exactly $w$.
\end{proof}


\begin{lemma} \label{lemma:carving-to-tree} Let $G$ be a graph with $\E{G} \neq \emptyset$. If $T$ is a carving-decomposition of $G$, then we can construct in polynomial time a tree-decomposition $(T, \chi)$ of $\Line{G}$ such that $width_t(T, \chi) = width_c(T) - 1$.
\end{lemma}
\begin{proof}
	Since $\E{G} \neq \emptyset$, $G$ must have at least two vertices and so $T$ has at least one arc. Fix an arbitrary arc $d \in \E{T}$. We can then define a function $next: \V{T} \rightarrow \E{T}$ by defining, for each $n \in \V{T}$, $next(n)$ to be the first edge along the (unique) shortest path from $n$ to $d$ (note if $n$ is adjacent to $d$ then we define $next(n) = d$).
	
	Then define $\chi: \V{T} \rightarrow 2^{\E{G}}$ by, for every node $m \in \E{T}$, define $\chi(m)$ to be the set of edges of $G$ shared between the subsets of vertices of $G$ induced by $T$ at $next(m)$. That is,
	$$\chi(m) \equiv \bigcap_{C \in \paritions{T, next(m)}} \vinc{G}{C}.$$
	
	We claim that $(T, \chi)$ is a tree-decomposition of $\Line{G}$. Note that $\V{\Line{G}} = \E{G}$ and so $\chi$ indeed labels the nodes of $T$ by subsets of vertices of $\Line{G}$. We can then check that the three properties of a tree-decomposition hold for $(T, \chi)$:
	\begin{enumerate}
		\item First, consider an arbitrary $e \in \V{\Line{G}}$. Since $e$ is an edge of $G$, $\einc{G}{e} \neq \emptyset$ and so let $v \in \einc{G}{e}$. Notice at $v$ is a leaf of $T$, and so the partitions induced by $T$ at $next(v)$ are $\{v\}$ and $\V{G} \setminus \{v\}$. Since $e$ is not a self-loop on $v$, $e$ is between these two sets of vertices and so $e \in \chi(v)$.
		
		\item Second, consider an arbitrary $\alpha \in \E{\Line{G}}$. Let $e$ and $f$ be the two vertices of $\Line{G}$ incident to $\alpha$. By definition of the line graph, $e$ and $f$ (as edges of $G$) must both be incident to some vertex $v \in \V{G}$. Thus both $e$ and $f$ are between $\{v\}$ and $\V{G} \setminus \{v\}$ and so both $e$ and $f$ are in $\chi(v)$. Thus $\einc{\Line{G}}{\alpha} \subseteq \chi(v)$.
		
		\item Finally, consider arbitrary nodes $n, o \in \V{T}$ and some arbitrary node $p \in \V{T}$ on the path from $n$ to $o$. Let $T_{n}$ be the subtree induced by $T$ at $next(n)$ that does not contain $p$, and similarly let $T_{o}$ be the subtree induced by $T$ at $next(o)$ that does not contain $p$. Finally, let $T_{p,1}$ and $T_{p,2}$ be the subtrees induced by $T$ at $next(p)$. Since $p$ is between $n$ and $o$, WLOG $T_{p,1}$ contains $n$ and $T_{p,2}$ contains $o$.
        
        It follows that $T_n$ is a subtree of $T_{p,1}$ and $T_o$ is a subtree of $T_{p,2}$. Thus $\chi(n) \subseteq \vinc{G}{\Lv{T_n}} \subseteq \vinc{G}{\Lv{T_{p,1}}}$ and $\chi(o) \subseteq \vinc{G}{\Lv{T_o}} \subseteq \vinc{G}{\Lv{T_{p,2}}}$. It follows that $\chi(n) \cap \chi(o) \subseteq \chi(p)$.
	\end{enumerate}
	
	Thus $(T, \chi)$ is indeed a tree-decomposition of $\Line{G}$. Moreover, the width of $T$ is given by
	\begin{align*}
    width_t(T, \chi) &= \max_{m \in \V{T}} | \chi(m) | - 1 \\
    &=  \max_{m \in \V{T}} \left| \bigcap_{C \in \paritions{T, next(m)}} \vinc{G}{C} \right| - 1 \\
    &= width_c(T) - 1,
    \end{align*}
	where the last equality holds since $next$ is surjective and $\paritions{T} = \bigcup_{a \in \E{T}} \paritions{T, a}$.
\end{proof}

% We focused on benchmarks from weighted model counting. The \emph{weighted model count} of $F$ (over propositional variables $X$) under weight functions $w^+, w^-: X \rightarrow \mathbb{R}$ is the sum over all solutions $Y$ to $F$ of $\prod_{y \in Y} w^+(y) \prod_{y \in X \setminus Y} w^-(y)$. It is straightforward to modify the reduction from model counting to tensor network contraction \cite{BMT15} to instead contract to the weighted model count of $F$. To do this, replace the copy tensor $\blacksquare_I$ corresponding to each variable $x$ by a weighted version: a tensor $\blacksquare_I' : \domain{I} \rightarrow \mathbb{C}$ that that maps the constant assignment $i \mapsto 1$ to $w^+(x)$, the constant assignment $i \mapsto 0$ to $w^-(x)$, and all other assignments $\tau \in \domain{I}$ to 0.

\subsection{Graph Decompositions}
\label{sec:prelim:decompositions}
In this work, we use two types of graph decompositions to find contraction orders for tensor networks: carving decompositions and tree decompositions. First, we describe carving decompositions \cite{ST94}, which we will use in Section \ref{sec:contraction-theory}:

\begin{definition}[Carving Decomposition]
	Let $G$ be a graph. A \emph{carving decomposition} of $G$ is an unrooted binary tree $T$ whose leaves are the vertices of $G$, i.e. $\Lv{T} = \V{G}$. 
	
    For every arc $a$ of $T$, deleting $a$ from $T$ yields exactly two trees, whose leaves define a partition of the vertices of $G$. Let $C_a \subseteq \V{G}$ be an arbitrary block of this partition. The \emph{width} of $T$ is the maximum number of edges in $G$ between $C_a$ and $\V{G} \setminus C_a$ for all $a \in \E{T}$, i.e.,
	$$width_c(T) = \max_{a \in \E{T}} \left| \vinc{G}{C_a} \cap \vinc{G}{\V{G} \setminus C_a} \right|.$$
    The width of a carving-decomposition $T$ with no edges is additionally defined to be 0.
\end{definition}
The \emph{carving width} of a graph $G$, notated $cw(G)$, is the minimum width across all possible carving decompositions of $G$. It is possible to find the carving width of a planar graph in time quadratic in the number of edges, but checking the carving width of an arbitrary graph is NP-Complete \cite{ST94}. 

Next, we define tree decompositions:
\begin{definition}[Tree Decomposition]
	Let $G$ be a graph. A \emph{tree decomposition} of $G$ is an unrooted binary tree $T$ together with a labeling function $\chi : \V{T} \rightarrow 2^{\V{G}}$ that satisfies the following three properties:
	\begin{enumerate}
		\item Every vertex of $G$ is contained in the label of some node of $T$. That is, $\V{G} = \bigcup_{n \in \V{T}} \chi(n)$.
		\item For every edge $e \in \E{G}$, there is a node $n \in \V{T}$ whose label is a superset of $\einc{G}{e}$, i.e. $\einc{G}{e} \subseteq \chi(n)$.
		\item If $n$ and $o$ are nodes in $T$, and $p$ is a node on the path from $n$ to $o$, then $\chi(n) \cap \chi(o) \subseteq \chi(p)$.
	\end{enumerate}
	The \emph{width} of a tree decomposition is the maximum size of the label of every node, minus 1. That is,
	$$width_t(T, \chi) = \max_{n \in \V{T}} | \chi(n) | - 1.$$
\end{definition}
The \emph{treewidth} of a graph $G$, notated $tw(G)$, is the minimum width across all possible tree decompositions of $G$. The treewidth of a tree is $1$, while the complete graph on $n$ vertices has treewidth $n-1$.

Tree decompositions have been widely applied across computer science \cite{MPPV04,GLST17}, and so a variety of heuristics and tools exist to find tree decompositions of low width. 
In Section \ref{sec:experiments}, we make use of two state-of-the-art heuristic solvers for tree decompositions: \textbf{Tamaki}, an unnamed solver \footnote{https://github.com/TCS-Meiji/PACE2017-TrackA} by H. Tamaki et. al, and \textbf{FlowCutter}, a solver\footnote{https://github.com/kit-algo/flow-cutter-pace17} by B. Strasser based on a graph-bisection algorithm \cite{HS18}. These solvers were respectively the first and second place solvers in the heuristic track of the PACE 2017 treewidth competition \cite{DKTW18}.

 (also called the \emph{covering graph}, \emph{representative graph}, \emph{edge graph}, etc.) 
 
 
 
\begin{lemma}
\label{lemma:network-contraction-partition-proof}
Let $M$ and $N$ be disjoint sets of tensors such that $M$, $N$, and $M \cup N$ are all tensor networks. Then $\tntensor{M \cup N} = \tntensor{M} \cdot \tntensor{N}$.
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma:network-contraction-partition}]
	No bound dimensions of $M$ appear in $N$ (and vice versa) since $M \cup N$ is a tensor network. Thus $\tnbound{M \cup N} = \tnbound{M} \sqcup \tnbound{N} \sqcup (\tnfree{M} \cap \tnfree{N})$. We can use this disjoint union to split the sum in the definition of $\tntensor{M \cup N}$ to see, for all $i \in \domain{\tnfree{M \cup M}}$, that    
	\begin{align*}
	&\tntensor{M \cup N}(i) = \sum_{j \in \domain{\tnbound{M \cup N}}} \prod_{A \in (N \cup M)} A((j \cup i)\restrict{\tdim{A}})\\
	 %&= \sum_{j \in \domain{\tnfree{M} \cap \tnfree{N}}} \sum_{k \in \domain{\tnbound{M}}} \sum_{l \in \domain{\tnbound{N}}} \prod_{A \in N} A((j \cup k \cup l \cup i)\restrict{\tdim{A}}) \prod_{B \in M} B((j \cup k \cup l \cup i)\restrict{\tdim{B}}) \\
	 &= \sum_{j \in \domain{\tnfree{M} \cap \tnfree{N}}} \left( \sum_{k \in \domain{\tnbound{M}}} \prod_{A \in N} A((j \cup k \cup i)\restrict{\tdim{A}}) \right)  \\
     &~~~~~~~~~~~~~~~~~~~~~~~~~\cdot ~~ \left(\sum_{l \in \domain{\tnbound{N}}} \prod_{B \in M} B((j \cup l \cup i)\restrict{\tdim{B}}) \right) \\
	 &= \sum_{j \in \domain{\tnfree{M} \cap \tnfree{N}}} \tntensor{M}(j \cup i\restrict{\tnfree{M}}) \cdot \tntensor{N}(j \cup i\restrict{\tnfree{N}}) \\
	 &= (\tntensor{M} \cdot \tntensor{N})(i).
	\end{align*}
\end{proof}

   % 	\begin{align*}
	%&\tntensor{M \cup N}(i) = \sum_{j \in \domain{\tnbound{M \cup N}}} \prod_{A \in (N \cup M)} A(j \cup i)\\
	%&= \sum_{\substack{j \in \domain{\tnfree{M} \cap \tnfree{N}}\\k \in \domain{\tnbound{M}}\\l \in \domain{\tnbound{N}}}} \prod_{A \in N} A(j, k, l, i) \prod_{B \in M} B(j, k, l, i) \\
	%&= \sum_{j \in \domain{\tnfree{M} \cap \tnfree{N}}} \left( \sum_{k \in \domain{\tnbound{M}}} \prod_{A \in N} A(j, k, i) \right) \\
    %&~~~~~~~~~~~~~~~~~~~~~~~~~~~\cdot\left(\sum_{l \in \domain{\tnbound{N}}}  \prod_{B \in M} B(j, l, i) \right) \\
	%&= \sum_{j \in \domain{\tnfree{M} \cap \tnfree{N}}} \tntensor{M}(j \cup i) \cdot \tntensor{N}(j \cup i) \\
	%&= (\tntensor{M} \cdot \tntensor{N})(i).
	%\end{align*}
    
    

\begin{lemma} \label{lemma:factorable-gives-tree}
Let $A$ be a fully-factorable tensor, let $T$ be a tree, and let $g: \tdim{A} \rightarrow \V{T}$ be a function such that $\Lv{T} \subseteq g(\tdim{A})$, i.e. every leaf of $T$ is in the range of $g$. Then there is a tensor contraction network $N$ with structure graph $G$ such that
\begin{enumerate}
\item $\tntensor{N} = A$,
\item $\max_{d \in \tnbound{N}} |\domain{d}| \leq \max_{e \in \tdim{A}} |\domain{e}|$, and
\item There is an isomorphism $h: \V{T} \rightarrow N$ between $T$ and $G \cap N$ with $d \in \tdim{h(g(d))}$ for all $d \in \tdim{A}$.
\end{enumerate}
\end{lemma}
\begin{proof}
By induction on $|\V{T}|$. If $|\V{T}| = 1$, then take $N = \{A\}$ and $h$ mapping the only node of $T$ to $A$.

Otherwise, assume $|\V{T}| \geq 1$ that this lemma holds for all trees of size $|T|-1$. Choose an arbitrary leaf $n \in \Lv{T}$ and let $D = g^{-1}(n)$. Since $n$ is in the range of $g$, $D \neq \emptyset$. Moreover, since $|\V{T}| \geq 1$ $T$ must have multiple leaves, and so $D \neq \tdim{A}$. Thus we can apply the definition of fully-factorable to obtain a fresh dimension $z$ and tensors $B$ and $C$ that satisfy the conditions of Definition \ref{def:fully-factorable}.

Let $o$ be the neighbor of $n$ in $T$. Construct $T'$ from $T$ by removing $n$ and the arc between $n$ and $o$. Observe that $C$ is fully-factorable and $\tdim{C} = (\tdim{A} \sqcup \{z\}) \setminus D$. Construct $g': \tdim{C} \rightarrow \V{T'}$ by mapping each $d \in \tdim{A} \setminus D$ to $g(d)$ and mapping $z$ to $o$. By the inductive hypothesis, we can apply Lemma \ref{lemma:factorable-gives-tree} to $C$ to get a tensor contraction network $N'$ and an isomorphism $h': \V{T'} \rightarrow N'$ such that $N'$ identifies $C$, every bound dimension of $N$ has domain smaller than the largest domain of $C$, and $d \in \tdim{h'(g'(d))}$ for all $d \in \tdim{C}$.

Let $N = N' \sqcup \{B\}$ and define $h: \V{T} \rightarrow N$ by $h = h' \sqcup \{n \mapsto B\}$. Then $\tntensor{N} = \tntensor{\{B\}} \cdot \tntensor{N'} = B \cdot C = A$ by Lemma \ref{lemma:network-contraction-partition}. Moreover, $\tnbound{N} = \tnbound{N'} \sqcup \{z\}$ and so condition 2 follows from condition 2 of Lemma \ref{lemma:factorable-gives-tree} and condition 3 of Definition \ref{def:fully-factorable}. Finally, $h$ is indeed an isomorphism since $h'$ was, and for all $d \in D$ we have $h(g(d)) = h(n) = B$ so $d \in \tdim{h(g(d))}$.
\end{proof}












let us construct a map $\vmap: H \rightarrow \V{T}$ to identify each vertex of $H$ to a node of $T$. 




If $\vmap(v)$ is a leaf node of $T$, define $\emap(v)$ to be the arc of $T$ incident to $\vmap(v)$. Otherwise, $\vmap(v)$ is an internal node of $T$. By construction, $v$ must therefore be a tensor of rank 2 or rank 3. If $v$ has rank $2$, since $h_A$ is an isomorphism there must be two other neighbors of $\vmap(v)$ that also contain $A$. Define $\emap(v)$ to be the arc between $\vmap(v)$ and an arbitrary one of these neighbors. 

It remains to define $\emap(v)$ for tensors $v$ of rank 3. Let 



For each leaf node $\ell \in \Lv{T}$, notice $|M_\ell| \leq 2$. If $|M_\ell| = 1$, replace $\ell$ in $S$ by the single element of $M_\ell$. Otherwise, add both elements of $M_\ell$ as new nodes in $S$ and add arcs from each element of $M_\ell$ to $\ell$. Observe that $\ell$ is no longer a leaf of $S$, and we have added all elements of $M_\ell$ as leaves of $S$.

Now, consider an internal node $n \in \V{T} \setminus \Lv{T}$. By construction, $M_n$ consists entirely of rank 2 and rank 3 tensors.

For each rank 2 tensor $h_A(n) \in M_n$, observe that $A$ must also be an element of the bag of two of the neighbors of $n$ (since $h_A$ is an isomorphism). Choose one such neighbor $m$ and let $a \in \vinc{S}{n}$ be the arc in the direction of $m$. We split $a$ in $S$ to attach $h_A(n)$ as a leaf. Now, consider the rank 3 tensors $h_A(n) \in M_n$. In a round-robin fashion, choose an arc of $\vinc{S}{n}$ and split it to attach $h_A(n)$ as a leaf. Observe that we have added all elements of $M_n$ as leaves of $S$.

We have now constructed a tree $S$ whose leaves consist of $\cup_n M_n = M$. Thus $S$ is a carving decomposition of $H$. Let us compute the width of $S$.

By construction, $\E{T} \subseteq \E{S}$. Consider an arc $a \in \E{T}$ between nodes $m, n \in \V{T}$. By construction, the edge separation induced by $a$ in $S$ is exactly $\chi(m) \cap \chi(n)$.  











If $|\tntensor{N}| = 3$ and $n$ has degree 3 in $T \cap V_f$, we treat the free vertex of $H$ as a rank 3 tensor and attach it in the same way.








Finally, if $|\tntensor{N}| = 3$, let $f$ be the free vertex of $G$. Observe that $T \cap V_f$ contains exactly one node $n$ of degree three. 



notice that $f_G$ 









Let $S_\ell$ be the graph whose vertices are $M_\ell$, with a single edge between the two vertices if $|M_\ell| = 2$. 
Begin with the tree $T$. 



We associate a tree $S_n$ to each node $n \in \V{T}$. For each leaf node $\ell \in \Lv{T}$, notice $|M_\ell| \leq 2$. Let $S_\ell$ be the graph whose vertices are $M_\ell$, with a single edge between the two vertices if $|M_\ell| = 2$. 

For each non-leaf node $n \in \V{T} \setminus \Lv{T}$, let $S_n$ be an arbitrary unrooted binary trees whose leaves are the elements of $M_n$ of degree 3 in $H$.

If $|\Lv{S_n}| = 1$


If $|\Lv{S_n}| \geq 3$, we additionally choose $s_n \in \V{S_n} \setminus \Lv{S_n}$ to be an internal node of $S_n$ such that there are no more than $\ceil{|\Lv{S_n}|/3}$ leaf nodes in each direction (such an internal node must always exist). Split each of the edges incident to $s_n$ to obtain a new set of three nodes, and associate each of the new nodes with one of the arcs $a \in \vinc{T}{n}$ in an arbitrary bijection.



For each of the three edges incident to $s_n$,



Choose an arbitrary bijection $h_n: \vinc{T}{n} \rightarrow \vinc{S_n}{s_n}$ between the arcs incident to $s$ and the arcs incident to $s_n$.

Finally, we link together these carving decompositions into a carving decomposition of $H$. For each arc $a \in T$ between $n, m \in T$, we add $a$ as an arc between $S_n$ and $S_m$. In particular, if $|\Lv{S_n}| \leq 2$ then we add a new node to $S_n$ in the middle of an arbitrary arc, while if $|\Lv{S_n}| \geq 3$ we add a new node to $S_n$ in



then we attach $a$ to the unique node of $S_n$, 


if $|\Lv{S_n}| \geq 3$ we add a new node in the middle of $h_n(a)$ and 






If we have chosen $s_n$ and $h_n$ for $S_n$, we introduce a new vertex on $h_n(a)$ and attach $a$ there (and similarly for $S_n$).






always a node  


There is always a node $s_n \in \V{S_n}$ that contains no more than $\ceil{|\Lv{S_n}|/3}$ leaf nodes on each side.




Choose a root $r \in \V{T}$ and, for each node $n \in V{T}$, define $C_n$ to be the union over $M_m$ over all $m \in \mathcal{C}(T, r, n)$. Observe that $C_r = N'$. We show by induction (on the distance 



First, we construct a carving decomposition associated to each node of $T$. Observe that each node $n \in \V{T}$ is associated with a set of tensors of $N'$ given by $M_n = \{ h_A(n) : A \in \chi(n) \cap N \}$, and let $G_n$ be the structure graph of $M_n$ without the free vertex. We construct a carving decomposition $S_n$ for $G_n$ as follows:
\begin{itemize}
\item For leaf nodes $\ell \in \Lv{T}$, notice that $M_\ell$ consists of two tensors (each of rank 1 or rank 2). Define $S_\ell$ to be the unique carving decomposition of $G_\ell$, and observe that its width is no larger than $|\chi(\ell)| = 2$. 
\item For non-leaf nodes $n \in \V{T} \setminus \Lv{T}$, notice that $M_n$ contains only rank 2 or rank 3 tensors. Partition the rank 3 tensors of $M_n$ into three sets $M^1_n$, $M^2_n$, and $M^3_n$ of size no more than $\ceil{|M_n|/3}$. For each $j \in \{1, 2, 3\}$, construct an arbitrary contraction tree $S^j_n$ for $M^j_n$ and observe that $S^j_n$ has max rank no more than $3 \ceil{|M_n|/3} \leq |M_n|+2$.
\end{itemize}



Observe that if $n$ is a leaf node then $C_n$ consists of two tensors (each of rank 1 or rank 2), while if $n$ is not a leaf node then all tensors in $C_n$ have rank 2 or rank 3.


% Let us begin by proving Lemma \ref{lemma:network-contraction-partition}, which we restate here:

%TODO: [Jeff] placement
% We say $C \subseteq \Lv{T}$ is a \emph{block induced by $T$} (resp. \emph{at $a$}) if $C$ is the set of leaves of some subtree of $T$ (resp. at $a$). We use $\paritions{T}$ to denote the set of partitions induced by $T$, and $\paritions{T,a}$ to denote the set of partitions induced by $T$ at $a$.

% If $G$ is a graph and $V \subseteq \V{G}$, we use $G \cap V$ to denote the subgraph of $G$ with $\V{G \cap V} = V$, $\E{G \cap V} = \{e \in \E{G}~:~\einc{G}{e} \cap V \neq \emptyset\}$, and $\einc{G \cap V}{e} = \einc{G}{e} \cap V$ for every $e \in \E{G \cap V}$. 

% and similarly if $E \subseteq \E{G}$ we define $\einc{G}{E} = \bigcup_{e \in E} \einc{G}{e}$
 
% Given an arc $a$ in a tree $T$, removing $a$ from $T$ partitions $T$ into two connected components, $T_1$ and $T_2$, both trees and subgraphs of $T$. The leaves of $T_1$ and $T_2$ are subsets of $\Lv{T}$. we call each component of such a partition a \emph{block induced by $T$}. We use $\blocks{T}$ to denote the set of blocks induced by $T$.

% 	Let $G$ be a graph. A \emph{carving decomposition} of $G$ is an unrooted binary tree $T$ whose leaves are the vertices of $G$, i.e. $\Lv{T} = \V{G}$. 
	
%     For each block $C$ induced by $T$, notice that $\{C, \V{G} \setminus C\}$ is a partition of the vertices of $G$. The \emph{width} of a carving-decomposition is the maximum number of edges in $G$ between $C$ and $\V{G} \setminus C$ across all blocks $C$ induced by $T$. That is,

